AE TextSpotter: Learning Visual and Linguistic Representation for Ambiguous Text Spotting

Scene text spotting aims to detect and recognize the entire word or sentence with multiple characters in natural images. It is still challenging because ambiguity often occurs when the spacing between characters is large or the characters are evenly spread in multiple rows and columns, making many visually plausible groupings of the characters (e.g. "BERLIN" is incorrectly detected as "BERL" and "IN" in Fig. 1(c)). Unlike previous works that merely employed visual features for text detection, this work proposes a novel text spotter, named Ambiguity Eliminating Text Spotter (AE TextSpotter), which learns both visual and linguistic features to significantly reduce ambiguity in text detection. The proposed AE TextSpotter has three important benefits. 1) The linguistic representation is learned together with the visual representation in a framework. To our knowledge, it is the first time to improve text detection by using a language model. 2) A carefully designed language module is utilized to reduce the detection confidence of incorrect text lines, making them easily pruned in the detection stage. 3) Extensive experiments show that AE TextSpotter outperforms other state-of-the-art methods by a large margin. For example, we carefully select a validation set of extremely ambiguous samples from the IC19-ReCTS dataset, where our approach surpasses other methods by more than 4%. The code has been released at https://github.com/whai362/AE_TextSpotter. The image list and evaluation scripts of the validation set have been released at https://github.com/whai362/TDA-ReCTS.

==> table/cmp_rs.tex <==
\begin{tabular}{l|c|c|c||c|c|c}
	\hline
	\multirow{2}{*}{Method} & \multicolumn{3}{c||}{Random-Sampling} & \multicolumn{3}{c}{TC-ReCTS} \\
	\cline{2-7}
	& Precision & Recall & F-Measure & Precision & Recall & F-Measure \\
	\hline
	EAST~[*] & & & & & \\
	% PMTD~[*] & & & & & \\
	PSENet~[*] & & & & & \\
	\hline
\end{tabular}


==> table/ic15.tex <==
\begin{tabular}{l|c|c|c|c|c|c|c|c}
	\hline
	\multirow{2}{*}{Method} & \multirow{2}{*}{Ext} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{Detection} & \multicolumn{3}{c}{End-to-End} \\
	\cline{4-9}
	& & & P & R & F & S & W & G  \\
	\hline
	TextNet~[*] & & & 89.4 & 85.4 & 87.4 & 78.7 & 74.9 & 60.5 \\
	He \emph{et al.}~[*] & & & 87 & 86 & 87 & 82 & 77 & 63 \\
	FOTS~[*] & \checkmark & ResNet50 & 91.0 & 85.2 & 88.0 & 81.1 & 75.9 & 60.8 \\
	Mask TextSpotter~[*] & \checkmark & ResNet50 & 91.6 & 81.0 & 86.0 & 79.3 & 73.0 & 62.4 \\
	Qin \emph{et al.}~[*] & \checkmark & ResNet50 & 89.4 & 85.75 & 87.5 & 83.4 & 80.0 & 68.0  \\
	\hline
	TCR TextSpotter w/o LM & \checkmark & ResNet50 & & & & & & \\
	TCR TextSpotter & \checkmark & ResNet50 & & & & & & \\
	\hline
\end{tabular}


==> table/lm_ab.tex <==
\begin{tabular}{l|c|c|c|c||c|c|c|c}
	\hline
	\multirow{2}{*}{Method} & \multicolumn{4}{c||}{All} & \multicolumn{4}{c}{Text Confusion Only} \\
	\cline{2-9}
	& Precision & Recall & F-Measure & * & Precision & Recall & F-Measure & * \\
	\hline
	w/o LM & & & & & & & \\
	w/ LM & & & & & & & \\
	\hline
\end{tabular}


==> table/lm_ab1.tex <==
\begin{tabular}{l|c|c|c|c}
	\hline
	Method & Precision & Recall & F-Measure & 1-NED  \\
	\hline
	w/o LM & 79.58 & 74.93 & 77.19 & \textcolor{red}{*}  \\
	w/ LM & 84.78 & 78.28 & 81.39 & \textcolor{red}{*} \\
	\hline
	Improve & +5.20 & +3.34 & +4.20 & \textcolor{red}{*} \\
	\hline
\end{tabular}


==> table/p_tc1.tex <==
\begin{tabular}{l|c|c|c|c|c||c|c|c}
	\hline
	 & \multicolumn{5}{c||}{Instance Level} & \multicolumn{3}{c}{Image Level} \\
	\cline{2-9}
	& Mixed & EN & CN & Num & Total & IC19 ReCTS & Total-Text & Total \\
	\hline
	Large & & & & & & & \\
	Multiple & & & & & & &  \\
	All & & & & & & 20000 & 1255 & 21255 \\
	\hline
\end{tabular}


==> table/rec.tex <==
\begin{tabular}{l|c}
	\hline
	Method & 1-NED \\
	\hline
	CRNN~[*] & 68.32 \\
	ASTER~[*] & 58.49 \\
	\hline
	CRM~(ours) & 71.21 \\
	\hline
\end{tabular}


==> table/rects_cmb.tex <==
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
	\hline
	\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{4}{c|}{IC19 ReCTS Testing Set} & \multicolumn{4}{c}{TC-ReCTS} \\
	\cline{3-10}
	& & P & R & F & NED & P & R & F & NED  \\
	\hline
	EAST~[*] & VGG16 & & & & - & & & & - \\
	PSENet~[*] & ResNet50 & 83.9 & 87.3 & 85.6 & - & 74.1 & 67.5 & 70.7 & - \\
	PMTD~[*] & ResNet50 & & & & - & & & & - \\
	FOTS~[*] & ResNet50 & & & & & & & & \\
	Mask TextSpotter~[*] & ResNet50 & 88.8 & 89.3 & 89.0 & 67.79 & 80.7 & 75.5 & 78.0 & \\
	\hline
	TCR TextSpotter w/o LM & ResNet50 & & & & & & \\
	TCR TextSpotter & ResNet50 & 91.5 & 92.1 & 91.8 & 71.8 & 83.6 & 79.1 & 81.3 & *** \\
	\hline
\end{tabular}


==> table/table1.tex <==
\begin{subtable}[t]{3.2in}
		% \setlength{\tabcolsep}{1.2mm}
		\begin{tabular}{l|c}
			\hline
			Method & Time Cost of $N$ Text Lines \\
			\hline
			CRNN~[*] & $20N$~ms \\
			ASTER~[*] & $30N$~ms \\
			CTRM~(ours) & $80 + 2N$~ms \\
			\hline
		\end{tabular}
	\caption{Todo.}
	\label{tab:k}
	% \vspace{5mm}
\end{subtable}
\quad
% loss
\begin{subtable}[t]{3.2in}
		\setlength{\tabcolsep}{1mm}
			\begin{tabular}{l|c|c|c|c}
				\hline
				Method & Precision & Recall & F-Measure & 1Gram  \\
				\hline
				w/o LM & 79.58 & 74.93 & 77.19 &  \\
				w/ LM & 84.78 & 78.28 & 81.39 & \\
				\hline
				Improve & +4.20 & +3.34 & +4.20 \\
				\hline
			\end{tabular}
	\caption{Todo.}
	\label{tab:faster_mask}
	% \vspace{5mm}
\end{subtable}

==> table/with_gt.tex <==
\begin{tabular}{c|c|c|c}
	\hline
	GT Char & P & R & F \\
	% & 1-NED  \\
	\hline
	$\times$ & 84.78 & 78.28 & 81.40 \\
	% & 51.32 \\
	$\surd$ & 87.48 & 78.62 & 84.81  \\
	% & 61.19  \\
	\hline
	Improve & \\
	\hline
\end{tabular}

